Complexity of the list homomorphism problem in hereditary graph classes

A homomorphism from a graph $G$ to a graph $H$ is an edge-preserving mapping from $V(G)$ to $V(H)$. For a fixed graph $H$, in the list homomorphism problem, denoted by LHom($H$), we are given a graph $G$, whose every vertex $v$ is equipped with a list $L(v) \subseteq V(H)$. We ask if there exists a homomorphism $f$ from $G$ to $H$, in which $f(v) \in L(v)$ for every $v \in V(G)$. Feder, Hell, and Huang [JGT~2003] proved that LHom($H$) is polynomial time-solvable if $H$ is a bi-arc-graph, and NP-complete otherwise. We are interested in the complexity of the LHom($H$) problem in graphs excluding a copy of some fixed graph $F$ as an induced subgraph. It is known that if $F$ is connected and is not a path nor a subdivided claw, then for every non-bi-arc graph the LHom($H$) problem is NP-complete and cannot be solved in subexponential time, unless the ETH fails. We consider the remaining cases for connected graphs $F$. If $F$ is a path, we exhibit a full dichotomy. We define a class called predacious graphs and show that if $H$ is not predacious, then for every fixed $t$ the LHom($H$) problem can be solved in quasi-polynomial time in $P_t$-free graphs. On the other hand, if $H$ is predacious, then there exists $t$, such that LHom($H$) cannot be solved in subexponential time in $P_t$-free graphs. If $F$ is a subdivided claw, we show a full dichotomy in two important cases: for $H$ being irreflexive (i.e., with no loops), and for $H$ being reflexive (i.e., where every vertex has a loop). Unless the ETH fails, for irreflexive $H$ the LHom($H$) problem can be solved in subexponential time in graphs excluding a fixed subdivided claw if and only if $H$ is non-predacious and triangle-free. If $H$ is reflexive, then LHom($H$) cannot be solved in subexponential time whenever $H$ is not a bi-arc graph.

==> intro-old.tex <==
Many natural graph-theoretic problems, including \textsc{Max Independent Set}, \textsc{$k$-Coloring}, \textsc{Max Cut}, \textsc{Min Odd Cycle Transversal}, etc., can be defined  in a uniform way as the question of the existence of certain graph homomorphisms.
For two graphs $G$ and $H$, a function $f : V(G) \to V(H)$ is a \emph{homomorphism from $G$ to $H$} if it maps edges of $G$ to edges of $H$, i.e., for every $uv \in E(G)$ it holds that $f(u)f(v) \in E(H)$. If $f$ is a homomorphism from $G$ to $H$ we denote it by $f : G \to H$.
As an important special case, we observe that if $H$ is a $k$-vertex clique, then homomorphisms to $H$ are precisely $k$-colorings of $G$. This is why homomorphisms to $H$ are often called \emph{$H$-colorings}.
We will refer to the graph $H$ as the \emph{target} and to the vertices of $H$ as \emph{colors}.
For a fixed graph $H$, by \homo{H} we denote the computational problem of deciding whether an instance graph $G$ admits a homomorphism to $H$.

The complexity dichotomy for the \homo{H} problem was shown by Hell and Ne\v{s}et\v{r}il~\cite{DBLP:journals/jct/HellN90}: If $H$ is bipartite or has a vertex with a loop, then the problem is polynomial-time-solvable, and otherwise it is \NP-complete.
The study of variants of graph homomorphisms has attracted a significant attention from the theoretical computer science community~\cite{DBLP:journals/tcs/Bulatov05,DBLP:journals/ejc/KunS16,DBLP:conf/lics/DalmauEHLR15,DBLP:conf/soda/EgriHLR14,DBLP:journals/dam/FederHSS11,DBLP:journals/siamdm/FederHKM03}.
Arguably, the most natural generalization of the problem is the \emph{list homomorphism problem}.
For a fixed graph $H$, an instance of the \lhomo{H} problem is a pair $(G,L)$, where $G$ is a graph and $L$ is a function that to every vertex $v \in V(G)$ assigns its \emph{$H$-list} (or \emph{list}, for short) $L(v) \subseteq V(H)$.
We ask if there exists a homomorphism $f : G \to H$, such that for every $v \in V(G)$ it holds that $f(v) \in L(v)$.
We write $f : (G,L) \to H$ to denote that $f$ is a list homomorphism from $G$ to $H$ which respects the lists $L$, and we write $(G,L) \to H$ to indicate that some such $f$ exists.

The complexity classification for \lhomo{H} was proven in three steps.
First, Feder and Hell~\cite{FEDER1998236} considered reflexive target graphs $H$, i.e., where every vertex has a loop.
In this case \lhomo{H} is polynomial-time solvable if $H$ is an interval graph and \NP-complete otherwise.
Then, Feder, Hell, and Huang~\cite{DBLP:journals/combinatorica/FederHH99} showed the dichotomy in the case that $H$ is irreflexive, i.e., has no loops. This problem appears to be polynomial-time solvable if $H$ is bipartite and its complement is a circular-arc graph, and \NP-complete otherwise.
Finally, Feder, Hell, and Huang~\cite{DBLP:journals/jgt/FederHH03} defined a new class of graphs with possible loops,
called \emph{bi-arc-graphs}, and showed that if $H$ is a bi-arc graph, then \lhomo{H} can be solved in polynomial time, and otherwise the problem is \NP-complete.
In case of reflexive graphs bi-arc graphs coincide with interval graphs, and in case of irreflexive graphs bi-arc graphs coincide with bipartite graphs whose complement is a circular-arc graph.
Let us point out that all mentioned hardness reductions for \lhomo{H} also exclude the existence of a subexponential-time algorithm, unless the ETH fails.

An active line of research is to study the complexity of computational problems, when the instance is assumed to belong some specific graph class. We usually assume that the considered classes are \emph{hereditary}, i.e., closed under vertex deletion. Each such a hereditary class can be characterized by a (possibly infinite) set of forbidden induced subgraphs.
For a family $\cF$ of graphs, a graph is \emph{$\cF$-free} if it does not contain any member of $\cF$ as an induced subgraph.
Most attention is put into considering classes with only one forbidden subgraph, i.e., for $\cF=\{F\}$.
In this case we write $F$-free, instead of $\{F\}$-free. We will always assume that $F$ is connected.

Let us define two important families of graphs. For an integer $t \geq 1$, by $P_t$ we denote the path with $t$ vertices.
For $a,b,c \geq 0$, by $S_{a,b,c}$ we denote the graph obtained by taking three disjoint paths $P_{a+1}$, $P_{b+1}$, and $P_{c+1}$ and merging one of the endvertices of each path into one vertex. Note that if at least one of $a,b,c$ is equal to 0, then $S_{a,b,c}$ is an induced path.
The members of $\{S_{a,b,c} ~|~ a,b,c \geq 0\}$ are called \emph{subdivided claws}. 

Let us briefly discuss the complexity of \textsc{$k$-Coloring} in $F$-free graphs.
First, we observe that if $F$ is not a path, then for every fixed $k \geq 3$,
the \textsc{$k$-Coloring} remains \NP-complete in $F$-free graphs.
Indeed, Emden-Weinert \emph{et al.} \cite{DBLP:journals/cpc/Emden-WeinertHK98} proved that the problem is hard for graphs with no cycles shorter than $p$, for any constant $p$.
Setting $p = |V(F)|+1$ yields the hardness for $F$-free graphs whenever $F$ contains a cycle.
On the other hand, \textsc{$k$-Coloring} is \NP-complete in line graphs~\cite{DBLP:journals/siamcomp/Holyer81a,DBLP:journals/jal/LevenG83}, which are in particular $S_{1,1,1}$-free.
This implies the hardness for $F$-free graphs if $F$ is a tree with maximum degree at least 3.
Combining these, we conclude that the only connected graphs $F$, for which we might hope for a polynomial-time algorithm for \textsc{$k$-Coloring} in $F$-free graphs, are paths.

The complexity of \textsc{$k$-Coloring} in $P_t$-free graphs has been an active area of research in the last two decades, see the survey by Golovach \emph{et al.}~\cite{DBLP:journals/corr/Golovach0PS14}.
The current state of art is as follows.
We know that for each fixed $k$, the problem is polynomial-time-solvable in $P_5$-free graphs~\cite{DBLP:journals/algorithmica/HoangKLSS10}.
On the other hand, for every $k \geq 5$, the problem is \NP-complete in $P_6$-free graphs~\cite{DBLP:journals/ejc/Huang16}.
The complexity of \textsc{4-Coloring} in $P_t$-free graphs is also fully understood: it is polynomial-time solvable for $t \leq 6$~\cite{DBLP:conf/soda/SpirklCZ19} and \NP-complete for $t \geq 7$~\cite{DBLP:journals/ejc/Huang16}.
Finally, we know that \textsc{3-Coloring} admits a polynomial time algorithm in $P_7$-free graphs~\cite{DBLP:journals/combinatorica/BonomoCMSSZ18}.
Interestingly, we know no proof of \NP-hardness of \textsc{3-Coloring} in $P_t$-free graphs, for any value of $t$.
The problem is believed to be solvable in polynomial time for every $t$, and obtaining such an algorithm is one of the main open questions in the area.

Let us point out that all mentioned hardness proofs rule out the existence of subexponential-time algorithms, unless the ETH fails.
Furthermore, all algorithmic results hold even for \textsc{List $k$-Coloring}, except for the case $(k,t)=(4,6)$, which is \NP-complete in the list setting~\cite{DBLP:journals/iandc/GolovachPS14}.

Even though our current toolbox seems to be insufficient to design a polynomial-time algorithm for \textsc{3-Coloring} $P_t$-free graphs for every fixed $t$, we can still solve the problem significantly faster than for general graphs.
Groenland \emph{et al.}~\cite{groenland2019h} showed that for every $t$, the problem can be solved in time $2^{\Oh(\sqrt{n \log n})}$ in $n$-vertex $P_t$-free graphs. Very recently, Pilipczuk, Pilipczuk, and Rz\k{a}\.zewski~\cite{pilipczuks-qpoly} observed that the breakthrough result by Gartland and Lokshtanov~\cite{DBLP:journals/corr/abs-2005-00690}, who showed a quasi-polynomial-time algorithm for the closely related \textsc{Max Independent Set} problem in $P_t$-free graphs, could be used to design an algorithm for \textsc{3-Coloring} with running time $n^{\Oh(\log^3 n)}$. They also presented an arguably simpler algorithm with running time $n^{\Oh(\log ^2n)}$.


The complexity of the \homo{H} and \lhomo{H} problems in $F$-free graphs received a lot less attention~\cite{DBLP:journals/dm/FederHH07,DBLP:journals/dam/KaminskiP19}.
Chudnovsky \emph{et al.}~\cite{DBLP:conf/esa/ChudnovskyHRSZ19} proved that if $F$ is not a subdivided claw, then for every relevant $k$ the \lhomo{C_k} problem remains \NP-complete and has no subexponential-time algorithm in $F$-free graphs.
This was later significantly generalized by Piecyk and Rz\k{a}\.zewski~\cite{piecyk}, as follows.
\begin{theorem}[Piecyk, Rzążewski~\cite{piecyk}] \label{thm:otherf}
Let $H$ be a fixed non-bi-arc graph.
If $F$ is connected and is not a subdivided claw,
then the $\lhomo{H}$ problem cannot be solved in time $2^{o(n)}$ in $n$-vertex $F$-free graphs, unless the ETH fails.
\end{theorem}

There are several results about the complexity of \lhomo{H} in $P_t$-free graphs.
First, Chudnovsky \emph{et al.}~\cite{DBLP:conf/esa/ChudnovskyHRSZ19} showed that for $k \in \{5,7,9\} \cup [10; \infty)$, the \lhomo{C_k} problem can be solved in polynomial time for $P_9$-free graphs.
Very recently, Chudnovsky \emph{et al.}~\cite{DBLP:conf/esa/ChudnovskyKPRS20} studied some further generalization of the homomorphism problem in subclasses of $P_6$-free graphs.
%Furthermore, the already mentioned $2^{\Oh(\sqrt{n \log n})}$-time algorithm by Groenland \emph{et al.}~\cite{groenland2019h} actually works for \lhomo{H} for a large family of graphs $H$: the requirement is that $H$ does not contain two vertices with two common neighbors.
%Later, Okrasa and Rz\k{a}\.zewski~\cite{DBLP:journals/jcss/OkrasaR20} observed that the same approach can be used to solve even more general \emph{weighted homorphism problem}, where in addition to lists we also have vertex- and edge-weights. They also proved that this more general problem cannot
%be solved in $P_t$-free graphs in subexponential time, whenever $H$ has two vertices with two common neighbors.
%However, for some of the hardness reductions it was essential to exploit the existence of vertex- and edge-weights and thus they cannot be translated to the arguably more natural \lhomo{H} problem.
Furthermore, the already mentioned $2^{\Oh(\sqrt{n \log n})}$-time algorithm by Groenland \emph{et al.}~\cite{groenland2019h} actually works  for \lhomo{H} for a large family of graphs $H$: the requirement is that $H$ does not contain two vertices with two common neighbors.
Even more generally, the algorithm can solve a \emph{weighted homomorphism problem}, where, in addition to lists, we allow vertex- and edge-weights.
Later, Okrasa and Rz\k{a}\.zewski~\cite{DBLP:journals/jcss/OkrasaR20} proved that the weighted homomorphism problem cannot
be solved in $P_t$-free graphs in subexponential time, whenever the target graph has two vertices with two common neighbors.
However, for some of the hardness reductions it was essential to exploit the existence of vertex- and edge-weights and thus they cannot be translated to the arguably more natural \lhomo{H} problem.


\paragraph{Our results.}
In this paper we investigate the fine-grained complexity of \lhomo{H} in $F$-free graphs, where $F$ is a subdivided claw.
Recall that by \cref{thm:otherf} these are the only connected forbidden graphs for which we can hope for the existence of subexponential-time algorithms.

First, we define the family of \emph{predacious} graphs, and show that they precisely correspond to ``hard'' cases of \lhomo{H} in $P_t$-free graphs. More specifically, we prove the following theorem.

\begin{theorem}\label{thm:ptfree-main}
Let $H$ be a fixed graph.
\begin{enumerate}[a)]
\item If $H$ is not predacious, then for every $t$,  the \lhomo{H} problem can be solved in time $n^{\Oh(\log^2 n)}$ in $n$-vertex $P_t$-free graphs.
\item If $H$ is predacious, then there exists $t$, such that the \lhomo{H} problem cannot be solved in time $2^{o(n)}$ in $n$-vertex $P_t$-free graphs, unless the ETH fails.
\end{enumerate}
\end{theorem}
Defining predacious graphs precisely requires introducing the decomposition theorem of target graphs $H$ by Okrasa \emph{et al.}~\cite{FullComplexity}, so we postpone it to \cref{sec:prelims}.
Roughly speaking, they are graphs that are simultaneously
non-bi-arc and contain a structure we call a \emph{predator}:
two vertices $a_1,a_2$ with two common neighbors $b_1,b_2$, such that $a_1$ and $a_2$ have incomparable neighborhoods and $b_1$ and $b_2$ have incomparable neighborhoods (i.e., the neighborhood of one vertex is not contained in the neighborhood of the other).
We remark that the definition of a predator is a refinement of the essential structure in the above-mentioned dichotomy for the weighted homomophism problem~\cite{groenland2019h,DBLP:journals/jcss/OkrasaR20}.

The proof of \cref{thm:ptfree-main}~a) builds on the decomposition of target graphs by Okrasa \emph{et al.}~\cite{FullComplexity} and on the recent quasi-polynomial-time algorithm for \textsc{3-Coloring} $P_t$-free graphs ~\cite{pilipczuks-qpoly}.
The hardness counterpart is proven in two steps. First, we consider a special case that $H$ is bipartite and ``undecomposable'' (the exact meaning of this is given in \cref{sec:prelims}). Okrasa \emph{et al.}~\cite{FullComplexity} analyzed the structure of such graphs and showed that it is rich enough to build a number of useful gadgets. We use them as building blocks of gadgets required in our hardness reduction.
Then, we lift this hardness result to general predacious graphs $H$, using the idea of \emph{associated bipartite graphs} introduced by Feder \emph{et al.}~\cite{DBLP:journals/jgt/FederHH03}.

\prz[inline]{update this section}

Next, we turn our attention to the case that $F$ is an arbitrary subdivided claw.
We obtain the dichotomy in two important special cases: that $H$ is irreflexive, and that $H$ is reflexive.
Recall that these two special cases correspond to the first two steps of the complexity dichotomy for \lhomo{H}~\cite{FEDER1998236,DBLP:journals/combinatorica/FederHH99}.

As a warm-up, let us discuss the case that $H$ is irreflexive and  $F$ is the simplest subdivided claw, i.e., the claw $S_{1,1,1}$.
Recall that \textsc{3-Coloring} is \NP-complete in line graphs~\cite{DBLP:journals/siamcomp/Holyer81a}, which are in particular claw-free.
Since the reduction yields an ETH lower bound, we obtain that if $H$ contains a simple triangle, then \lhomo{H} cannot be solved in subexponential time in claw-free graphs (observe that every instance of \lhomo{K_3} can be seen as an instance of \lhomo{H}, where the other vertices of $H$ do not appear in any lists).

So let us consider the case that $H$ is triangle-free. We note that there is no homomorphism $K_3 \to H$, so if the instance graph contains a triangle, we can immediately report a no-instance. On the other hand, $\{S_{1,1,1},K_3\}$-free graphs are just collections of disjoint paths and cycles, where the problem can be solved in polynomial time using  dynamic programming.
We generalize this simple classification to the case if $F$ is an arbitrary subdivided claw as follows.

\begin{theorem}\label{thm:subdividedclaw-irreflexive}
Let $H$ be a fixed irreflexive graph.
\begin{enumerate}[a)]
\item If $H$ is non-predacious and triangle-free, then for every $a,b,c$,  the \lhomo{H} problem can be solved in time $2^{\Oh(\sqrt{n \log n})}$ in $n$-vertex $S_{a,b,c}$-free graphs.
\item If $H$ is predacious or contains a triangle, then there exist $a,b,c$, such that the \lhomo{H} problem cannot be solved in time $2^{o(n)}$ in $n$-vertex $S_{a,b,c}$-free graphs, unless the ETH fails.
\end{enumerate}
\end{theorem}

The algorithm from \cref{thm:subdividedclaw-irreflexive}~a) is based on the existence of the so-called \emph{extended strip decomposition}~\cite{DBLP:journals/combinatorica/ChudnovskyS10}.
Very recently, a similar approach was used by Chudnovsky \emph{et al.}~\cite{chudnovsky2020quasi} to obtain a QPTAS and a subexponential-time algorithm for the \textsc{Max Independent Set} problem in $S_{a,b,c}$-free graphs.
However, the decomposition itself is not structured enough to be useful for coloring problems, such as \lhomo{H}.

So we proceed as follows. First, similarly as before, we can restrict ourselves to instances that are $\{S_{a,b,c},K_3\}$-free.
We carefully analyze the structure of such graphs $G$ and show that they admit a refined extended strip decomposition, with much simpler structure.
Very roughly speaking, we can find a ``small'' set $X \subseteq V(G)$, such that for each connected component $C$ of $G - X$, the vertices of $C$ can be partitioned into ``small'' sets called \emph{atoms}, that can be arranged in a path-like or cycle-like manner.
We exhaustively guess the coloring of $X$ (which is fine, as $X$ is small). For each atom we can solve the problem recursively.
Finally, we use the path-like or cycle-like arrangement of atoms to combine partial results using dynamic programming,
similarly as we did in the case of $\{S_{1,1,1},K_3\}$-free graphs.

Let us point out that the assumption that $H$ is irreflexive and triangle-free is only used to ensure that the instance is triangle-free.
For such instances we can solve \lhomo{H} in subexponential time for \emph{every} non-predacious graph $H$.

The hardness counterpart of \cref{thm:subdividedclaw-irreflexive} is simple.
If $H$ is predacious, then we are done by \cref{thm:ptfree-main}~b), as every $P_t$-free graph is also $S_{t,t,t}$-free.
On the other hand, if $H$ contains a simple triangle, then the problem is hard even in claw-free graphs, as mentioned before.

Finally, we show that if $H$ is reflexive, then the only ``easy'' cases are the ones that are polynomial-time solvable in general graphs.

\begin{theorem}\label{thm:subdividedclaw-reflexive}
For every fixed reflexive non-bi-arc graph $H$, there exist $a,b,c$, such that the \lhomo{H} problem cannot be solved in time $2^{o(n)}$ in $n$-vertex $S_{a,b,c}$-free graphs, unless the ETH fails.
\end{theorem}

Unfortunately, we were not able to provide the full complexity dichotomy for $S_{a,b,c}$-free graphs.
We conjecture that the distinction between ``easy'' and ``hard'' cases is as follows.

\begin{restatable}{conjecture}{conj}
\label{conj}
%\begin{conjecture}
Assume the ETH. Let $H$ be a non-bi-arc graph.
Then for all $a,b,c$, the \lhomo{H} problem can be solved in time $2^{o(n)}$ in $n$-vertex $S_{a,b,c}$-free graphs
if and only if none of the following conditions is satisfied:
\begin{enumerate}
\item $H$ is predacious,
\item $H$ contains a simple triangle,
\item $H$ contains two incomparable vertices with loops.
\end{enumerate}
%\end{conjecture}
\end{restatable}


\paragraph{Organization of the paper.} In \cref{sec:prelims} we present some notation and preliminary results. In particular, we define the class of predacious graphs. In \cref{sec:ptfree} we prove \cref{thm:ptfree-main}: the algorithmic statement in  \cref{sec:ptfree-algo} and the hardness counterpart in \cref{sec:ptfree-hardness}.
In \cref{sec:subdivided} we consider $S_{a,b,c}$-free graphs.
In \cref{sec:subdivided-algo} we prove \cref{thm:subdividedclaw-irreflexive}~a) and in \cref{sec:subdivided-hardness} we present some hardness results, which, in particular, imply \cref{thm:subdividedclaw-irreflexive}~b) and \cref{thm:subdividedclaw-reflexive}.
In \cref{sec:conclusion} we revisit our hardness results and discuss the minimum size of the forbidden graph $F$, for which the \cref{thm:ptfree-main}~b), \cref{thm:subdividedclaw-irreflexive}~b), and \cref{thm:subdividedclaw-reflexive} hold. We also discuss and motivate \cref{conj}.


==> line-graphs.tex <==
For a graph $G$, we say that edge $xy \in V(G)$ is a \emph{pending edge}, if $\deg_G(x)=1$. 
In the next hardness proof (\cref{thm:line-graphs-two-loops}) we are going to consider the class of line graphs, which form a particular subclass of $S_{1,1,1}$-free graphs. 
However, to simplify the argument that the instance we construct is a line graph, instead of constructing gadgets which are instances $(G,L)$ of \lhomo{H}, we will construct graph $G$ and \emph{edge-lists} $L:E(G) \to H$ so that $(\cL(G),L)$ is an instance of \lhomo{H}.
We call such pair $(G,L)$ an \emph{edge instance}.
Therefore, if $(G,L)$ is an edge instance, and $(\cL(G),L)$ is some gadget we already defined (e.g., $\rneq(S)$-gadget), we call the edges corresponding to the interface vertices of the gadget \emph{interface edges}.\prz{żeby to miało sen, interface vertex musi być stopnia 1, nie?}
\ko{na tym etapie wciąż chyba ma sens tak, nie?}
%Moreover, when building such an instance, instead of identifying some vertices of introduced parts of the constructed graph, we will sometimes need to identify edges. 

We define the operation of identifying two pending edges of two respective graphs as follows.
Consider two edge instances $(G_1,L_1),(G_2,L_2)$, and two pending edges $x_1y_1 \in E(G_1)$, $x_2y_2 \in E(G_2)$ (w.l.o.g. assume that $\deg_{G_1}(x_1)= \deg_{G_2}(x_2)=1$) such that $L(x_1y_1)=L(x_2y_2)$. 
By identifying the edges $x_1y_1$ and $x_2y_2$ we mean constructing an edge instance $(G,L)$ by taking a copy of $(G_1,L)$ and $(G_2,L)$, removing vertices $x_1$ and $x_2$, and adding an edge $y_1y_2$ with $L(y_1y_2)=L(x_1y_1)$. 

Before we proceed to the reduction, we construct some arbitrary gadget, which will be useful in the construction.
\begin{lemma}\label{lem:half-edge-gadget-path}
Let $H$ be a connected, non-bi-arc graph, such that $H^*$ is undecomposable.
Let $u_0,u_1 \in V(H)$ be incomparable vertices with loops, such that $u_0u_1 \notin E(H)$.
Then there exists an edge instance $(P(u_0,u_1),L)$ such that $P(u_0,u_1)$ is a path on at least four vertices with two pending edges $x_1,x_2$ for which $L(x_1)=L(x_2)=\{u_0,u_1\}$, and the following holds:
\begin{enumerate}[1.]
\item there exists $h_0: (\cL(P(u_0,u_1)),L) \to H$ such that $h_0(x_1)=u_0$ and $h_0(x_2)=u_1$,
\item there exists $h_1: (\cL(P(u_0,u_1)),L) \to H$ such that $h_1(x_1)=u_1$ and $h_1(x_2)=u_0$, 
\item there is no $h: (\cL(P(u_0,u_1)),L) \to H$ such that $h(x_1)=h(x_2)=u_0$.
\end{enumerate}
% a $\rneq(\{u_1,u_2\})$-gadget, whose interface vertices are pending edges of~$G$. 
\end{lemma}
\begin{proof}
Since $u_0,u_1$ are incomparable in $H$, sets $\{u'_0,u'_1\}$ and $\{u''_0,u''_1\}$ are incomparable in $H^*$.
Let $\alpha, \beta \in V(H^*)$ be as in \cref{thm:distinguisher}, without loss of generality we assume that they belong to the same bipartition class as $u'_0$ and $u'_1$.

By \cref{thm:distinguisher} we obtain $(D^{\alpha/\beta}_{u'_0/u'_1},L')$ and $(D^{\beta/\alpha}_{u'_0/u'_1},L')$. 
Denote by $x_1$ and $x_2$, respectively, the $x$-vertices of paths $D^{\alpha/\beta}_{u'_0/u'_1}$ and $D^{\beta/\alpha}_{u'_0/u'_1}$ (so $L(x_1)=L(x_2)=\{u'_0,u'_1\}$).
Also, denote by $y_1$ and $y_2$, respectively, the $y$-vertices of paths $D^{\alpha/\beta}_{u'_0/u'_1}$ and $D^{\beta/\alpha}_{u'_0/u'_1}$ (so $L(x_1)=L(x_2)=\{\alpha,\beta\}$).
We construct $(D,L')$ by identifying the vertices $y_1$ and $y_2$ into $y$.
Clearly, $D$ is a path with endvertices $x_1,x_2$. 

Due to the properties of $(D^{\alpha/\beta}_{u'_0/u'_0},L')$ and $(D^{\beta/\alpha}_{u'_0/u'_1},L')$, is straightforward that
(i) there exist $h_0: (D,L') \to H^*$ such that $h_0(x_1)=u'_0$ and $h_0(x_2)=u'_1$, and
(ii) there exist $h_1: (D,L') \to H$ such that $h_1(x_1)=u'_1$ and $h_1(x_2)=u'_0$, and
(iii) there is no $h: (D,L') \to H$ such that $h(x_1)=h(x_2)=u'_0$.
% $(D,L')$ is an $\rneq(\{u'_1,u'_2\})$-gadget (see \cref{fig:edge-gadget-path}).
Finally, we for every $x \in V(D)$ define $L(x):= \{a ~|~ \{a',a''\} \cap L'(x) \neq \emptyset\}$.
By \cref{lem:homo-star} we have $(D,L') \to H^*$ if and only if $(D,L) \to H$, therefore $(D,L)$ must satisfy the properties listed in the statement of the lemma.
We take $P(u_0,u_1)$ to be the path such that $\cL(P(u_0,u_1))=D$.
\end{proof}

We show that \cref{lem:half-edge-gadget-path} can be used to prove a strengthening of \cref{lem:edge-gadget} when $S$ has only two special elements.

\begin{corollary}\label{cor:edge-gadget-path}
Let $H$ be a connected, non-bi-arc graph, such that $H^*$ is undecomposable.
Let $u_0,u_1 \in V(H)$ be incomparable vertices with loops, such that $u_0u_1 \notin E(H)$.
Then there exists an edge instance $(G,L)$ such that $(\cL(G),L)$ is a $\rneq(\{u_0,u_1\})$-gadget, whose interface vertices are pending edges of~$G$.
\end{corollary}
\begin{proof}
We first construct $G'$ by taking two paths $P(u_0,u_1)$ and $P(u_1,u_0)$, obtained by \cref{lem:half-edge-gadget-path}. 
Let $v^0_1,v^0_2$ and $v^1_1,v^1_2$, respectively, be the endvertices these paths.
We identify $v^0_1$ with $v^1_1$, creating $v_1$. 
We identify $v^0_2$ with $v^1_2$, creating $v_2$.
Note that both $P(u_0,u_1)$ and $P(u_1,u_0)$ have more that one edge, therefore, we do not create parallel edges.
Moreover, properties 1.-3. of \cref{lem:half-edge-gadget-path} for $P(u_0,u_1)$ and $P(u_1,u_0)$ ensure that we created an instance such that $(\cL(G'),L)$ is a $\rneq(\{u_0,u_1\})$-gadget, with two arbitrary edges adjacent in $G$ to $v_1$ and $v_2$, respectively, as interface vertices.
Observe that now it is enough to add vertices $v'_1$ and $v'_2$ and pending edges $v_1'v_1$ and $v_2v'_2$ such that $L(v_1'v_1)=L(v_2v'_2)=\{u_0,u_1\}$ to obtain the desired gadget.
\end{proof}

%\begin{figure}
%\begin{center}
%\tikzstyle{vertv}=[draw,circle,fill=white,inner sep=0pt,minimum size=30pt]
%\tikzstyle{nooo}=[draw=none,fill=none,inner sep=0pt]
%\begin{tikzpicture}[scale=0.8]
%\draw[line width=3,gray!50] (-2,0) -- (0,0);
%\draw[line width=3,gray!50] (7.5,0) -- (9.5,0);
%%\draw[line width=3,gray!50] (6.3,1.2) -- (3.7,1.2);
%
%\draw[color=gray!20,rounded corners=17pt,rotate=18,fill=gray!20,fill opacity=0.3] (-.6,.6) rectangle (4.5,-.6) {};
%\draw[color=gray!20,rounded corners=17pt,rotate=-18,fill=gray!20,fill opacity=0.3] (-.6,.6) rectangle (4.5,-.6) {};
%%%%druga strona
%\begin{scope}[xshift=7.5cm,yscale=1,xscale=-1]
%\draw[color=gray!20,rounded corners=17pt,rotate=18,fill=gray!20,fill opacity=0.3] (-.6,.6) rectangle (4.5,-.6) {};
%\draw[color=gray!20,rounded corners=17pt,rotate=-18,fill=gray!20,fill opacity=0.3] (-.6,.6) rectangle (4.5,-.6) {};
%\end{scope}
%\node[vertv,label=left:\footnotesize{$x'$}] at (-2,0) {};
%\node[vertv,label=right:\footnotesize{$y'$}] at (9.5,0) {};
%\node[vertv,label=above:\footnotesize{$x=x^1=x^3$}] at (0,0) {};
%\node[vertv,label=below:\footnotesize{$y_3=y_4$}] at (3.7,-1.2) {};
%\node[vertv,label=above:\footnotesize{$y_1=y_2$}] at (3.7,1.2) {};
%\node[vertv,label=above:\footnotesize{$y=x^2=x^4$}] at (7.5,0) {};
%\node[nooo] at (7.5,0.25) {\footnotesize{$u'_2$}};
%\node[nooo] at (7.5,-.25) {\footnotesize{$u'_1$}};
%\node[nooo] at (9.5,0.25) {\footnotesize{$u'_2$}};
%\node[nooo] at (9.5,-.25) {\footnotesize{$u'_1$}};
%
%\node[nooo] at (0,0.25) {\footnotesize{$u'_1$}};
%\node[nooo] at (0,-.25) {\footnotesize{$u'_2$}};
%
%\node[nooo] at (-2,0.25) {\footnotesize{$u'_1$}};
%\node[nooo] at (-2,-.25) {\footnotesize{$u'_2$}};
%
%\node[nooo] at (3.7,1.45) {\footnotesize{$\alpha$}};
%\node[nooo] at (3.7,0.95) {\footnotesize{$\beta$}};
%
%\node[nooo] at (3.7,-1.45) {\footnotesize{$\alpha$}};
%\node[nooo] at (3.7,-0.95) {\footnotesize{$\beta$}};
%
%\draw[blue] (0.15,0.4) -- (3.4,1.45);
%\draw[blue] (0.15,-0.3) -- (3.6,.8);
%\draw[red] (0.15,0.4) -- (3.6,.8);
%
%\draw[blue] (0.15,-0.3) -- (3.4,-1.45);
%\draw[blue] (0.15,0.4) -- (3.6,-.8);
%\draw[red] (0.15,-0.3) -- (3.6,-.8);
%
%\draw[blue] (-.15,0.4) -- (-1.85,0.4);
%\draw[blue] (-.15,-.3) -- (-1.85,-.3);
%\draw[red] (-.15,0.4) -- (-1.85,-.3);
%\draw[red] (-.15,-.3) -- (-1.85,0.4);
%
%\begin{scope}[xshift=7.5cm,yscale=1,xscale=-1]
%\draw[blue] (0.15,0.4) -- (3.4,1.45);
%\draw[blue] (0.15,-0.3) -- (3.6,.8);
%\draw[red] (0.15,-0.3) -- (3.4,1.45);
%
%\draw[blue] (0.15,-0.3) -- (3.4,-1.45);
%\draw[blue] (0.15,0.4) -- (3.6,-.8);
%\draw[red] (0.15,0.4) -- (3.4,-1.45);
%
%\draw[blue] (-.15,0.4) -- (-1.85,0.4);
%\draw[blue] (-.15,-.3) -- (-1.85,-.3);
%\draw[red] (-.15,0.4) -- (-1.85,-.3);
%\draw[red] (-.15,-.3) -- (-1.85,0.4);
%\end{scope}
%\end{tikzpicture}
%\end{center}
%\caption{A schematic view of the construction of graph $D$ from the proof of \cref{lem:edge-gadget-path}.}
% \label{fig:edge-gadget-path}
%\end{figure}
%Rozbiłam na dwa lematy i teraz chyba już nie trzeba obrazka

We finally proceed to the proof of the theorem. A \emph{walk} $\cA$ is a sequence $\cA =a_1,\ldots, a_\ell$ of vertices of graph $G$, such that for every $i \in [\ell-1]$ we have $a_ia_{i+1} \in E(G)$.
%Walk $\cA =a_1,\ldots, a_\ell$ \emph{avoids} walk $\cB =b_1,\ldots, b_\ell$ on the same number of elements if $a_1 \neq b_1$ and for every $i \in [\ell-1]$ it holds that $a_ib_{i+1} \not\in E(G)$.
%By $\cC_\ell(u)$ we denote the \emph{constant} walk $u,u,\ldots,u$ of length $\ell$.

%For a family $\mathbb{S}=\{\cA_1,\ldots,\cA_q\}$ of walks of length $\ell$, we denote by $(P(\mathbb{S}),L)$ the edge instance such that $P(\mathbb{S})$ is a path on $\ell+1$ vertices and the lists $L$ of the consecutive edges of $P(\mathbb{S})$ consists of consecutive elements of walks from $\mathbb{S}$.
%Observe that if we have two walks $\cA_1=a_1,\ldots,a_\ell$ and $\cA_2=a'_1,\ldots,a'_\ell$ such that $\cA_1$ avoids $\cA_2$, then 

\begin{theorem}\label{thm:line-graphs-two-loops}
Let $H$ be a connected undecomposable, non-bi-arc graph. 
Assume that $H^*$ contains an induced cycle $C$ on at least 6 vertices, and there exist $u_0,u_1 \in V(H)$ with loops such that $u_0u_1 \not\in E(H)$, $u_0'u_0'' \in E(C)$, and $\{u'_1,u''_1\} \cap V(C) \neq \emptyset$. 
Then the $\lhomo{H}$ problem cannot be solved in time $2^{o(n)}$ in line graphs, unless ETH fails.
\end{theorem}
\begin{proof}
%If possible, choose $C$ in a way that $u_1',u_1'' \in V(C)$ (i.e., $u_1'u_1''$ is an edge of $C$). 
%Then we choose the smallest cycle out of the possible ones.
%Without loss of generality we assume that $u_1'$ belongs to $C$.
Denote by $\ell \geq 6$ the number of vertices of $C$ and denote its consecutive vertices by $x'_0,x_1'',x_2',\ldots,x''_{\ell-1}$. 
Without loss of generality we assume that $x_0=x_1=u_0$. 
Let $i \in [2,\ell-1]$ be such $x_i=u_1$.
Actually, note that since $u_0u_1 \notin E(H)$, we must have $i \in [3,\ell-2]$. 

\begin{claim}\label{cla:walks}
There exist (not necessarily distinct) vertices $v_0,v_1 \in N(u_1)$ such that $v_0v_1 \not\in E(H)$. Moreover, for $i=0,1$ there exist walk $\cA_i:~u_1 \to v_i$, such that only its last element belongs to $N(u_0)$.
\end{claim}
\begin{proof}[Proof of claim]
We define $v_0=x_2$ and $v_1=x_{\ell-1}$.
Observe that $v_0v_1 \notin E(H)$, since $C$ is an induced cycle on at least 6 vertices, and $x_2' \not\in N(x_{\ell-1}'')$. 
Moreover, as $C$ is an induced cycle, for every $j \in [3,\ell-2]$ we have $x_j \notin N(u_0)$, as otherwise we would have $x'_jx''_0 \in E(C)$ or $x''_jx'_1 \in E(C)$.
This implies that walks 
$\cA_0= u_1, x_{i-1}, x_{i-2}, \ldots, x_2$, and $\cA_1= u_1, x_{i+1}, x_{i+2}, \ldots, x_{\ell-1}$ satisfy the statement of the claim.
\end{proof}

First, we construct the edge instance $(F,L)$, such that $(\cL(F),L)$ is an $\textrm{OR}_3(u_1,u_2)$-gadget whose interface vertices are pending edges of $F$.
Let $v_0,v_1,\cA_0$, and $\cA_1$ be as in \cref{cla:walks}, and let $\ell_0$ and $\ell_1$ be, respectively, the number of elements of $\cA_0$ and $\cA_1$. 
Denote the consecutive vertices of $\cA_1$ and $\cA_2$, respectively, by $a_1,a_2,\ldots, a_{\ell_1}$ and $a'_1,a'_2,\ldots, a'_{\ell_2}$.
Clearly, we can assume that for every $i < \ell_0$ (resp. $i < \ell_1$) we have $a_i \neq v_0$ (resp. $a'_i \neq v_1$), as otherwise we can choose shorter path.
Note that $a_1=a'_1=u_1$, $a_{\ell_1}=v_0$, and $a_{\ell_2}=v_1$.

For $i \in \{0,1\}$ let $P_i=p^i_1,p^i_2,\ldots,p^i_{\ell_i+1}$ be a path.
We define its edge lists as $L(p^0_jp^0_{j+1})=\{u_0,a_j,u_1\}$ for every $j \in [\ell_0]$ and $L(p^1_jp^1_{j+1})=\{u_0,a'_j,u_1\}$ for every $j \in [\ell_1]$. 
We also take $P_2$ to be the path $P(u_1,u_0)$ with endvertices $y_1$ and $y_2$ obtained by \cref{lem:half-edge-gadget-path}.

\begin{claim}For $i=0,1$, the mapping $h:\{p^i_1p^i_2,p^i_{\ell_i} p^i_{\ell_i+1}\} \to \{u_0,u_1,v_i\}$ can be extended to homomorphism $(\cL(P_i),L)$ if and only if $(h(p^i_1p^i_2),h(p^i_{\ell_i} p^i_{\ell_i+1})) \in \{(u_0,u_0), (u_1,u_1),(u_0,v_i),(u_1,v_i)\}$.
\end{claim}

We obtain edge instance $(F,L)$ by identifying vertices $p^1_{\ell_0+1}$, $p^2_{\ell_1+1}$ and $y_2$ into one vertex (so that $F$ is isomorphic to $S_{\ell_0,\ell_1,\ell_2}$, where $\ell_2$ is the number of vertices of $P_2$ minus one).

\begin{claim}\label{cla:or-gadget}
$(\cL(F),L)$ is an $\textrm{OR}_3(u_1,u_2)$-gadget with pending edges of $F$ as interface vertices.
\end{claim}
 
The final step of the proof is a straightforward reduction from 3-\sat. 
Consider a formula $\Phi$ of 3-\sat with variables $x_1,\ldots, x_N$ and clauses $C_1,\ldots,C_M$. 
For every $i \in [N]$ let $p_N$ denote the number of occurrences of the literal $x_i$ in the clauses. 
Without loss of generality we can assume that each clause has exactly three literals.

We construct a graph $G^*$ and lists $L: E(G^*) \to 2^{V(H)}$, such that $(\cL(G^*),L)$ is an instance of \lhomo{H}.
First, for every $i \in [N]$ we introduce a star $S_i$ with a center $z^i$ and $p_i$ leaves $z^i_1,\ldots,z^i_{p_i}$. 
These leaves correspond to the occurrences of the variable $x_i$.
For every $e \in E(S_i)$ we set $L(e)=\{u_1,u_2\}$.
Note that since $u_1u_2 \notin E(H)$, all edges in a single star must be mapped to the same vertex.
Then, for every negated occurrence of $x_i$ we add graph $G$ constructed by \cref{cor:edge-gadget-path}, such that $(\cL(G),L)$ is a $\textrm{NEQ}(\{u_1,u_2\})$-gadget with interface edges $s_1$ and $s_2$. If $v^i_j$, for some $j \in [p_i]$ is a vertex corresponding to such occurrence, we identify edges $v^iv^i_j$ and edge $s_1$ of the corresponding $\textrm{NEQ}(\{u_1,u_2\})$-gadget.
Therefore, for $j$-th occurrence of variable $x_i$, we have a corresponding \emph{literal edge}, which is $z^iz^i_j$ for the positive occurrence, and $s_2$ (of the corresponding $\textrm{NEQ}(\{u_1,u_2\})$-gadget) for the negative occurrence.

Last, for every clause $C_i$ we add graph $F$ constructed before, such that $(\cL(F),L)$ is an $\textrm{OR}_3(u_1,u_2)$-gadget by \cref{cla:or-gadget} and identify its interface edges with corresponding literal edges.  
It is straightforward to verify that $(G^*,L) \to H$ if and only if $\Phi$ admits a satisfying assignment.
\end{proof}

==> subdivided-claw-esd.tex <==
In this section we focus on the class of $S_{a,b,c}$-free graphs. 
First, in \cref{sec:algo-irreflexive} we present a subexponential-time algorithm for $\{S_{a,b,c},K_3\}$-free graphs.
This serves as a main tool in the proof of the algorithmic statement in \cref{thm:subdividedclaw-irreflexive}.
Then, in \cref{sec:subdivided-hardness} we discuss the hard cases.
In particular, we complete the proof of \cref{thm:subdividedclaw-irreflexive} and show \cref{thm:subdividedclaw-reflexive}.

\subsection{Subexponential-time algorithm for $\{S_{a,b,c},K_3\}$-free graphs}\label{sec:subdivided-algo}

To describe the algorithm, we first need to introduce the notion of an \emph{extended strip decomposition}~\cite{DBLP:journals/combinatorica/ChudnovskyS10,chudnovsky2020quasi}.
For a graph $G$, by $T(G)$ we denote the set of all triangles in $G$, i.e., three-element sets $\{x,y,z\}$ of pairwise adjacent vertices.
Similarly as we write $xy$ for an edge $\{x,y\}$, we will denote a triangle $\{x,y,z\}$ shortly by $xyz$.

Let $G$ be a simple graph. An \emph{extended strip decomposition} $(D, \eta)$ of $G$ consists of:
\begin{itemize}
\item a simple graph $D$,
\item a set $\eta(x) \subseteq V(G)$ for every $x \in V(D)$,
\item a set $\eta(xy) \subseteq V(G)$ for every $xy \in E(D)$, and subsets $\eta(xy,x),\eta(xy,y) \subseteq \eta(xy)$,
\item a set $\eta(xyz) \subseteq V(G)$  for every $xyz \in T(D)$,
\end{itemize}
which satisfy the following properties:
\begin{enumerate}
\item $\{\eta(o)~|~o \in V(D)\cup E(D) \cup T(D)\}$ is a partition of $V(G)$,
\item for every $x \in V(D)$ and every distinct $y,z \in N_D(x)$, the set $\eta(xy,x)$ is complete to $\eta(xz,x)$,
\item every $uv \in E(G)$ is contained in one of the sets $\eta(o)$ for $o \in V(D) \cup E(D)\cup T(D)$ or is as follows:
\begin{itemize}
\item $u \in \eta(xy,x), v\in \eta(xz,x)$ for some $x \in V(D)$ and $y,z \in N_D(x)$, or
\item $u \in \eta(xy,x), v\in \eta(x)$ for some $xy \in E(D)$, or
\item $u \in \eta(xyz)$ and $v\in \eta(xy,x) \cap \eta(xy,y)$ for some $xyz \in T(D)$. 
\end{itemize}
\end{enumerate}
We will sometimes refer to elements of $V(D) \cup E(D) \cup T(D)$ as \emph{objects} of $D$.

We distinguish some subsets of $V(G)$ which are called \emph{atoms} of a decomposition $(D,\eta)$. 
For an object  $o \in V(D) \cup T(D)$, the set $\eta(o)$ is called a \emph{vertex atom} or a \emph{triangle atom}, accordingly.
Now consider $xy \in E(D)$.
The set $\eta(xy) \setminus \left(\eta(xy,x) \cup \eta(xy,y)\right)$ is called an \emph{edge interior atom}.
The set $\eta(x) \cup \eta(xy) \setminus \eta(xy,y)$ is called a \emph{half-edge atom}.
Finally, the set $\eta(x) \cup \eta(y) \cup \eta(xy) \cup \bigcup_{xyz \in T(D)} \eta(xyz)$ is called a \emph{full edge atom}.

Note that for each $o \in V(D)\cup E(D) \cup T(D)$, the set $\eta(o)$ is contained in at least one atom
(to be more specific, $\eta(o)$ is always contained in some vertex atom or some full edge atom).
If $A$ is an atom of $(D,\eta)$, we write $A \in (D,\eta)$. We also define $\alpha(D,\eta) :=\max_{A \in (D,\eta)}|A|$.


Let us first show the following simple technical claim about extended strip decompositions of disconnected graphs.
\begin{lemma} \label{lem:esd-disconnected}
Let $G$ be a graph and let $(D,\eta)$ be its extended strip decomposition.
Then in polynomial time we can obtain an extended strip decomposition $(D',\eta')$, such that (i) $\alpha(D',\eta') \leq \alpha(D,\eta)$, (ii)
for each connected component $C$ of $D'$, the set $\bigcup_{o \in V(C) \cup E(C) \cup T(C)} \eta'(o)$ contains the vertices of exactly one connected component of $G$, and (iii) $G$ and $D'$ have the same number of connected components.
\end{lemma}
\begin{proof}
Suppose there is a set $S \subseteq V(G)$, such that $G[S]$ is a connected component of $G$, and for some connected component $C$ of $D$
it holds that 
\[
S \cap \left( \bigcup_{o \in V(C) \cup E(C) \cup T(C)} \eta(o) \right) \neq \emptyset \quad \text{ and } \quad (V(G) \setminus S) \cap \left( \bigcup_{o \in V(C') \cup E(C') \cup T(C')} \eta(o) \right) \neq \emptyset.
\]
Introduce to $D$ a copy of $C$ (the sets $\eta(o)$ are also copied).
Now, in one copy of $C$, we remove from all sets $\eta(o)$ for objects of $C$ all vertices of $S$,
and in another copy we remove all vertices of $V(G) \setminus S$. Repeating this step exhaustively yields the extended strip decomposition satisfying properties (i) and (ii).

For (iii), observe that for each connected component $G[S]$ of $G$, the vertices of $S$ might appear in sets $\eta(o)$ for objects
of exactly one connected component of $D'$. This is because for distinct connected components $C,C'$ of $D'$,
there are no edges in $G$ between $\bigcup_{o \in V(C) \cup E(C) \cup T(C)} \eta(o)$ and $\bigcup_{o \in V(C') \cup E(C') \cup T(C')} \eta(o)$.
Thus, if the number of components of $D'$ is larger than the number of components of $G$, there must exist components $C$ of $D'$, such that  
$\bigcup_{o \in V(C) \cup E(C) \cup T(C)} \eta(o) = \emptyset$. Clearly, we can safely remove such components from $D'$.
\end{proof}



We observe that if $G$ is simple and triangle-free, then, given an extended strip decomposition of $G$,
we can simplify it significantly without increasing the maximum atom size.

\begin{lemma}\label{lem:triangle-free-esd}
Let $G$ be a connected triangle-free graph and let $(D,\eta)$ be an extended strip decomposition of $G$,
such that $D$ is connected.
Then there exists a extended strip decomposition $(D', \eta')$ of $G$ such that:
%\begin{multicols}{2}
\begin{enumerate}[(1)]
\item for every atom $A \in (D', \eta')$ we have $|A| \leq \alpha(D,\eta)$, \label{it:decomp-size}
\item $\eta'(xyz) = \emptyset$ for every $xyz \in T(D')$, \label{it:decomp-triangle}
\item $D'$ is a simple graph with maximum degree at most 2, \label{it:decomp-degree}
\item if for some edge $xy$ of $D'$ we have $\eta'(xy,x)=\emptyset$, then $x$ is of degree 1 in $D'$. \label{it:decomp-leaf}
\end{enumerate}
Furthermore, $(D', \eta')$ can be found in polynomial time.
%\end{multicols}
\end{lemma}

\begin{proof}
Let $\alpha := \alpha(D,\eta)$. We say that an object $o \in V(D) \cup E(D) \cup T(D)$ is \textit{trivial} if $\eta(o)=\emptyset$. 
Also, we say that $xy \in E(D)$ is \textit{$x$-trivial} if $\eta(xy,x)=\emptyset$.
First, observe that if only one object $o \in V(D) \cup E(D) \cup T(D)$ is non-trivial, then $|V(G)|\leq \alpha$,
as the set $\eta(o)$ is contained in some atom of $(D,\eta)$.
In this case a decomposition where $V(D') = \{x\}$ and $\eta'(x)=V(G)$ satisfies the statement of the lemma.

Note that the above case applies in particular when some non-trivial edge $xy \in E(D)$ is both, $x$- and $y$-trivial.
Indeed, in such a case, since the only neighbors of $\eta(xy)$ that might have neighbors outside this set are in $\eta(xy,x) \cup \eta(xy,y)$,
we have a contradiction with $G$ being connected.

So from now on we will assume that there are at least two non-trivial objects in $D$.
Note that since $G$ is connected, at least one of these objects must be an edge of $D$.
In particular, this implies that $D$ has at least two vertices.
Let us first analyze some properties of $(D,\eta)$ that are implied by triangle-freeness of $G$.

\begin{claim}\label{cl:atmosttwoedges}
For each $x \in V(D)$ there are at most two edges adjacent to $x$ which are not $x$-trivial.
\end{claim}
\begin{claimproof}
If there are distinct $y,y',y'' \in N_D(x)$ such that $\eta(xy,x),\eta(xy',x)$, and $\eta(xy'',x)$ are non-empty,
then any vertices $v \in \eta(xy,x)$, $v' \in \eta(xy',x)$, and $v'' \in \eta(xy'',x)$ form a triangle in $G$, a contradiction.
\end{claimproof}

\begin{claim} \label{cl:triangleatmosttwo} 
For any $xyz \in T(D)$, at most two of the sets $\eta(xy,x) \cap \eta(xy,y)$, $\eta(yz,y) \cap \eta(yz,z)$, and $\eta(xz,x) \cap \eta(xz,z)$ are non-empty.
\end{claim}
\begin{claimproof}
Any three vertices $u \in \eta(xy,x) \cap \eta(xy,y)$, $v \in \eta(yz,y) \cap \eta(yz,z)$, and $w \in \eta(xz,x) \cap \eta(xz,z)$
form a triangle in $G$, a contradiction.
\end{claimproof}

\begin{claim} \label{cl:triangleatleastone}
For any $xyz \in T(D)$, if all sets  $\eta(xy,x) \cap \eta(xy,y)$, $\eta(yz,y) \cap \eta(yz,z)$, and $\eta(xz,x) \cap \eta(xz,z)$ are empty,
then the triangle $xyz$ is trivial. 
\end{claim}
\begin{claimproof}
For contradiction, suppose otherwise. Observe that there no edge from $\eta(xyz)$ to $V(G) \setminus \eta(xyz)$,
and since $V(G) \setminus \eta(xyz)$ is non-empty, $G$ is disconnected.
\end{claimproof}

\medskip
We will modify $(D,\eta)$ into $(D',\eta')$ in two steps.
First, let us define an intermediate decomposition which satisfies property \cref{it:decomp-triangle}.

By \cref{cl:triangleatmosttwo} and \cref{cl:triangleatleastone},
we can introduce the following classification of non-trivial triangles in $xyz \in T(D)$.
If exactly one of $\eta(xy,x) \cap \eta(xy,y)$, $\eta(yz,y) \cap \eta(yz,z)$, and $\eta(xz,x) \cap \eta(xz,z)$ is non-empty,
we say that $xyz$ is of type~1.
Otherwise, i.e., if two of these sets are non-empty, we say that $xyz$ is of type~2. 

We will construct a mapping $\sigma$ from non-trivial triangles of $D$ to $V(D) \cup E(D)$.
For a non-trivial triangle $xyz \in T(D)$, we define $\sigma(xyz)$ as follows:
\begin{itemize}
\item $\sigma(xyz) := xy$ if $xyz$ is of type~1 and $N(\eta(xyz)) \subseteq \left(\eta(xy,x) \cap \eta(xy,y)\right)$,
\item $\sigma(xyz) : = x$ if $xyz$ is of type 2 and $N(\eta(xyz)) \subseteq \left(\eta(xy,x) \cap \eta(xy,y)\right) \cup \left(\eta(xz,x) \cap \eta(xz,z)\right)$.
\end{itemize} 
Note that since two intersecting edges can belong to only one triangle, no two triangles are mapped to the same vertex $x \in V(D)$.

We define a new extended strip decomposition $(D,\eta'')$ of $G$ as follows.
For each $o \in V(D) \cup E(D)$, we define
\[\eta''(o) := \eta(o) \cup \bigcup_{xyz \in T(D), \text{ s.t. } \sigma(xyz)=o} \eta(xyz).\]
For each $xy \in E(D)$, we set $\eta''(xy,x):=\eta(xy,x)$.
Finally, for each $xyz \in T(D)$, we define $\eta''(xyz):=\emptyset$.
Intuitively speaking, each set associated with a non-trivial triangle $xyz$ of $D$ has been absorbed into the set associated with the object $\sigma(xyz)$.

It is straightforward to verify that $(D,\eta'')$ is an extended strip decomposition of $G$ and it clearly satisfies property \cref{it:decomp-triangle}. Let us now discuss the sizes of atoms in $(D,\eta'')$.
Observe that it is sufficient to consider full edge atoms, as every other non-empty atom is contained in some full edge atom (recall that $D$ has at least one edge and is connected).


%Consider $x \in V(D)$ and its vertex atom $\eta''(x)$.\prz{czy to potrzebne?}
%If there is no triangle $xyz \in T(D)$, such that $\sigma(xyz)=x$, then $|\eta''(x)|=|\eta(x)| \leq \alpha$.
%Otherwise, recall that there is exactly one triangle $xyz$ with $\sigma(xyz)=x$, and $\eta''(x) = \eta(x) \cup \eta(xyz)$.
%Note that this atom is contained in the full edge atom of $(D,\eta)$ associated with the edge $xy$, i.e., $\eta(x) \cup \eta(y) \cup \eta(xy) \cup \bigcup_{xyz' \in T(D)} \eta(xyz')$. This implies that $|\eta''(x)| \leq \alpha$.


So consider a full edge atom $A'$ of $(D,\eta'')$ for an edge $xy \in E(D)$,
i.e., $A'=\eta''(x) \cup \eta''(xy) \cup \eta''(y) \cup \bigcup_{xyz' \in T(D)}\eta''(xyz')$.
%Clearly, $\eta''(xyz) =\emptyset$ for every $xyz \in T(D)$, so $A=\eta''(x) \cup \eta''(xy) \cup \eta''(y)$.
We claim that if $xy$ is neither $x$-trivial nor $y$-trivial, then $|A'| \leq \alpha$.
Clearly, $\bigcup_{xyz' \in T(D)}\eta''(xyz')=\emptyset$, so $A'=\eta''(x) \cup \eta''(xy) \cup \eta''(y)$.
Let $A$ be a full-edge atom of $(D,\eta)$ associated with $xy$.

First, note that for each triangle $xyz$, such that $\eta(xyz) \subseteq \eta''(xy)$ (or, equivalently, $\sigma(xyz)=xy$)
we always have $\eta(xyz) \subseteq \bigcup_{xyz' \in T(D)}\eta(xyz') \subseteq A$.
Apart from such triangles, $\eta''(xy)$ contains only the vertices from $\eta(xy)$, so since  $\eta(xy) \subseteq A$, we have $\eta''(xy) \subseteq A$.

So if $\eta''(x)=\eta(x)$ and $\eta''(y)=\eta(y)$, then $\eta''(x) \cup \eta''(y)$ is also contained in $A$,
which implies $|A'| \leq |A|\leq  \alpha$.
Otherwise, assume that $\eta''(x) \neq \eta(x)$ (the case $\eta''(y) \neq \eta(y)$ is analogous).
This means that there is a triangle $xzz' \in T(D)$, which is of type~2 and $\sigma(xzz') = x$.
%
By the definition of $\sigma$, this means that $N_G(\eta(xzz')) \subseteq \left(\eta(xz,x) \cap \eta(xz,z) \right) \cup  \left(\eta(xz',x) \cap \eta(xz',z')\right)$, and $\eta(xz,x) \cap \eta(xz,z) \neq \emptyset$, $\eta(xz',x) \cap \eta(xz',z') \neq \emptyset$.
%
In particular, both edges $xz$ and $xz'$ are not $x$-trivial.
Therefore, as we assumed that $xy$ is not $x$-trivial, by \cref{cl:atmosttwoedges} we have $y\in \{z,z'\}$. 
This implies that $\eta(xyz) \subseteq A$ and thus $\eta''(x) \subseteq A$. Hence $|A'| \leq |A| \leq \alpha$. 

%Now consider a half-edge atom $A$ for $x \in V(D)$ and $xy \in E(D)$, i.e., $A=\eta''(x) \cup \eta''(xy) \setminus \eta''(xy,y)$.
%Recall that $\eta''(xy) = \eta(xy) \cup \bigcup_{xyz \in T(D), \text{ s.t. } \sigma(xyz)=xy} \eta(xyz)$.
%First, consider the case that $\eta''(x) = \eta(x)$, i.e., there is no non-trivial triangle $o$, such that $\sigma(o)=x$.
%In this case $A$ is contained in the full edge atom of $(D,\eta)$ associated with $xy$, and thus $|A| \leq \alpha$. 

%So now consider the case that $\eta''(x) \neq \eta(x)$. This means that there is exactly one triangle $o \in T(D)$, such that $\sigma(x) = o$.
%If this triangle contains the edge $xy$, then again we conclude that $A$ is contained in the full edge atom of $(D,\eta)$ associated with $xy$, and thus $|A| \leq \alpha$.
%So finally assume that $o = xzz'$, where $y \notin \{z,z'\}$. This means that $x$ has three distinct neighbors $y,z,z'$.
%Furthermore, from the definition of type~2, we know that the sets $\eta(xz,z) \cap \eta(xz,x)$ and $\eta(xz',x) \cap \eta(xz',z')$ are both non-empty, so both edges $xz$ and $xz'$ are not $z$-trivial. By \cref{cl:atmosttwoedges} this implies that the edge $xy$ is $x$-trivial.

Summing up, we have shown that the only full edge atoms of $(D,\eta'')$ that might violate property \cref{it:decomp-size}
are the ones associated with some edge $xy$, which is $x$-trivial, and $x$ is in some triangle of $D$.
In particular, $x$ is of degree at least 2.
We will say that for some $xy \in E(D)$ the pair $(xy,x)$ is \emph{bad} if $xy$ is $x$-trivial and $x$ is of degree at least 2.

\medskip
Now we will modify $(D,\eta'')$ into yet another extended strip decomposition of $G$,
which satisfies all properties listed in the statement of the lemma.
Consider a bad pair $(xy,x)$. We modify $D$ as follows.
We remove the edge $xy$ from $E(D)$, and add a new vertex $x'$ and the edge $x'y$.
We extend $\eta''$ by setting $\eta''(x'y):=\eta''(xy)$, $\eta''(x'y,y) := \eta''(xy,y)$, and $\eta''(x') = \eta(x'y,x'):=\emptyset$.
Since $N(\eta(x'y)) \subseteq \eta(y)$, this is still an extended strip decomposition of $G$.

Note that the number of bad pairs decreased by one. 
We repeat this step exhaustively, let $(D',\eta')$ be the final extended strip decomposition obtained this way.

It is clear that $(D',\eta')$ satisfies property \cref{it:decomp-triangle}.
If $D'$ has a vertex of degree $x$ at least $3$, then, by \cref{cl:atmosttwoedges}, for at least one neighbor $y$ of $x$ we have that $xy$ is $x$-trivial. Thus $(xy,x)$ is a bad pair, which violates the definition of $(D',\eta')$, so the property \cref{it:decomp-degree} holds.
Similarly we conclude that the property \cref{it:decomp-leaf} holds as well.

Finally, note that when defining $\eta$ we did not increase the sizes of any atoms, compared to to $\eta''$.
Furthermore, recall that the only full edge atoms that could violate property \cref{it:decomp-size} in $(D,\eta'')$ are full edge atoms associated with some edge $xy$, where $(xy,x)$ is a bad pair. Since in the last step we removed all bad pairs edges $xy$,
and every atom is contained in some full edge atom, we conclude that property \cref{it:decomp-size} holds as well.
\end{proof}


We will also need the following structural result of Chudnovsky \emph{et al.}~\cite{chudnovsky2020quasi},
which says how extended strip decompositions relate to the class of graphs we are considering.

\begin{lemma}[Chudnovsky \emph{et al.}~\cite{chudnovsky2020quasi}]\label{lem:sttt-free-decomposition}
Let $t \geq 4$, let $G$ be a connected $S_{t,t,t}$-free graph on $n$ vertices,
and let $\sigma \in (0, \frac{1}{100t})$ be such that  
for every $v \in V(G)$ we have $N[v] \leq \sigma^8 \cdot n$.
Then there exists $X \subseteq V(G)$ and an extended strip decomposition of $G \setminus X$,
such that $\alpha(D,\eta) \leq (1-\sigma^7)n$ and $|X| \leq \sigma (n-\alpha(D,\eta))$.
Furthermore, this decomposition can be found in polynomial time.
\end{lemma}

Combining \cref{lem:esd-disconnected}, \cref{lem:triangle-free-esd}, and \cref{lem:sttt-free-decomposition}, we obtain the following corollary.

\begin{corollary}\label{cor:final-esd}
Let $a,b,c$ be constants and let $n$ be sufficiently large.
Let $G$ be a connected $\{S_{a,b,c},K_3\}$-free graph on $n$ vertices with $\Delta(G) < n^{1/9}$.
Then there exists $X \subseteq V(G)$ and an extended strip decomposition $(D,\eta)$ of $G \setminus X$, such that:
\begin{enumerate}[(1)]
\item $\alpha(D,\eta) \leq n-n^{2/9}$, \label{it:decomp-size-cor}
\item $|X| \leq n^{-1/9} (n-\alpha(D,\eta))$, \label{it:decomp-sizeX-cor}
\item $\eta(xyz) = \emptyset$ for every $xyz \in T(D)$,
\item $D$ is a simple graph with maximum degree at most 2, 
\item if for some edge $xy$ of $D$ we have $\eta(xy,x)=\emptyset$, then $x$ is of degree 1 in $D$, \label{it:decomp-leaf-cor}
\item there is a bijection $f$ between connected components of $G-X$ and connected components of $D$,
so that the vertices of each connected component $C$ of $G-X$ are contained in the union of sets $\eta(o)$ over the objects of $f(C)$.
\end{enumerate}
Furthermore, this decomposition can be found in polynomial time.
\end{corollary}

\begin{proof}
Set $t := \max (a,b,c,4)$, $\sigma := n^{-1/9}$, and assume that $n$ is large enough so that $\sigma < \frac{1}{100t}$.
Observe that $G$ is $S_{t,t,t}$-free.

We first apply \cref{lem:sttt-free-decomposition} to obtain a set $X$ and an extended strip decomposition $(D',\eta')$ of $G-X$.
Note that they satisfy the first two conditions.
Using \cref{lem:esd-disconnected}, we modify $(D',\eta')$ into a new extended strip decomposition $(D'',\eta'')$ satisfying the first two and also the last condition.
Finally, we apply \cref{lem:triangle-free-esd} to each pair $(C,f(C))$, where $C$ is a connected component of $G - X$ and $f$ is the bijection given in the last condition, and obtain the decomposition $(D,\eta)$.
It is clear that it satisfies all required properties.
\end{proof}


\begin{theorem} \label{thm:subdivided-claw-free-algo}
Let $H$ be a connected graph which does not contain a predator.
Then for every $a,b,c\geq 0$, the \lhomo{H} problem can be solved in time $2^{\Oh(n^{8/9} \log n)}$ in $n$-vertex $\{S_{a,b,c},K_3\}$-free graphs.
\end{theorem}
\begin{proof}
Clearly we can assume that $n$ is sufficiently large, as otherwise we can solve the problem by exhaustive enumeration.
In the proof we will present a recursive algorithm. Let $F(n)$ be the running time bound on instances with $n$ vertices.
We aim to show that there is a constant $a$, such that $F(n) \leq |V(H)|^{a \cdot n^{8/9} \log n} = 2^{\Oh(n^{8/9} \log n)}$.

Each step of the algorithm begins with a preprocessing phase, in which we exhaustively apply the following three reduction rules, in given order:
(i) for every $v \in V(G)$, if there exist distinct $a,b \in L(v)$ such that $N_H(a) \subseteq N_H(b)$, then remove $a$ from $L(v)$, 
(ii) for every $v \in V(G)$ and $a \in L(v)$, if there exists $u \in N_G(v)$ such that $N_H(a) \cap L(u) = \emptyset$,  then remove $a$ from $L(v)$, and 
(iii) for every $v \in V(G)$, if $|L(v)|=1$, then remove $v$ from $G$.
The correctness of the rules (i) and (ii) is straightforward, and for the rule (iii), notice that by (ii) the lists of all neighbors of $v$ contain only neighbors of the element of $L(v)$. 
If after these steps any list is empty, there is no way to properly color $G$ with lists $L$, so we immediately terminate and report a no-instance.
Otherwise, we may assume that every list is an incomparable set, has at least two elements,
and for every $uv \in E(G)$ and for every $a \in L(v)$ there exists $b \in L(u)$ such that $ab \in E(H)$. 
Clearly the preprocessing step can be performed in polynomial time.

In the algorithm we consider two cases.
First, suppose that exists a vertex $v \in V(G)$ such that $\deg_G(v)\geq n^{1/9}$.
It implies that there exists a list $L'$ assigned to at least $\ell:=n^{1/9}/2^{|V(H)|}$ neighbors of $v$. 
By \cref{obs:branching-works} there exist $a\in L(v)$ and $b\in L'$ such that $ab \not\in E(H)$.
We branch on assigning $a$ to $v$; either we remove $a$ from $L(v)$ or color $v$ with $a$ and remove $b$ from the lists of all neighbors of $v$.
Note that in the latter case at least $\ell$ lists are affected.
The complexity of this step is described by the following recursive inequality, where $N := \sum_{v \in V(G)} |L(v)|$:
\[
\widetilde{F}(N) \leq \widetilde{F}(N-1) + \widetilde{F}(N- \ell) \leq \ell^{\Oh(N/\ell)}.
\]
As $N \leq |V(H)| \cdot n$ and $\ell = n^{1/9}/2^{|V(H)|}$, we obtain that the complexity $F(n)$ in this case is $F(n) = n^{\Oh(n^{8/9})} \leq |V(H)|^{a \cdot  n^{8/9} \log n}$, provided that $a$ is sufficiently large.


\bigskip
Now consider the case that the degree of every vertex in $G$ is smaller than $n^{1/9}$. 
Applying \cref{cor:final-esd} to $G$  yields a set $X \subseteq V(G)$ and an extended strip decomposition $(D,\eta)$ of $G-X$, satisfying the conditions stated in the corollary. In particular, we have $\alpha:=\alpha(D,\eta) \leq n - n^{2/9}$ and $|X| \leq n^{-1/9}(n - \alpha)$, every connected component of $D$ is a path or a cycle, and all triangle atoms are empty.

Before we proceed to the description of the second step of the algorithm, let us discuss one more property of $(D,\eta)$.
Consider a vertex $x$ of $D$ with degree 2, let its neighbors be $y$ and $z$.
By property \cref{it:decomp-leaf-cor} in \cref{cor:final-esd} we know that $\eta(xy,x) \neq \emptyset$ and $\eta(xz,x) \neq \emptyset$.
Recall that the set $\eta(xy,x)$ is complete to $\eta(xz,x)$. This implies that the size of each of these sets is smaller than $n^{1/9}$,
as otherwise $G$ would contain a vertex of degree at least $n^{1/9}$.

We proceed as follows. First, we exhaustively guess the colors of vertices of $X$ (we only consider colorings $(G[X],L|_X) \to H$).
There are at most $|V(H)|^{|X|} \leq |V(H)|^{n^{-1/9}(n - \alpha)}$ possibilities .
Suppose that we are in one of the branches;  we need to decide whether the coloring of $X$ can be extended to remaining vertices of $G$.
First, we adjust the lists of vertices in $V(G) \setminus X$, so that they are consistent with the coloring of $X$.
More precisely, for an edge $uv \in E(G)$, such that $u \in X$ and $v \notin X$, we remove from $L(v)$ every non-neighbor of the color of $u$.
This can clearly be done in polynomial time. To simplify the notation, we will still denote the updated lists by $L$.
Now we can forget about the vertices of $X$ and the whole problem is reduced to solving the instance of \lhomo{H} on the graph $G \setminus X$.
Note that the problem can be solved independently for each connected component of $G$, and we report a yes-instance if all components are yes-instances.
So let us consider a connected component $G'$ of $G \setminus X$, and the connected component $D'$ of $D$, which corresponds to $G'$.
For brevity, we will still use $\eta$ to denote this function restricted to objects of~$D'$.

The following claim is the heart of our algorithm.

\begin{claim}\label{cl:extend}
We can solve the instance $(G',L)$ of \lhomo{H} in time $|V(H)|^{4n^{1/9}} \cdot F(\alpha) \cdot n^{\Oh(1)}$.
\end{claim}
\begin{claimproof}
Recall that $D'$ is a path or a cycle. 
We will also distinguish one more special case, that $D'$ is a path with at most two vertices.
We deal with the three cases separately.

\paragraph{Case 1: $D'$ has at most two vertices.}
In this case all vertices of $G'$ are contained in one atom of $D'$ -- either a vertex atom, if $D'$ is a single vertex, or a full edge atom, if $D'$ has two vertices. In both cases \cref{cor:final-esd}~\cref{it:decomp-size-cor} implies that $|V(G')| \leq \alpha$.
We call the algorithm recursively for $(G',L)$ and it solves the subproblem in time $F(\alpha)$.

\paragraph{Case 2: $D'$ is a path with at least two edges.}
Denote the consecutive vertices of $D'$ by $x_1, \ldots, x_{m+2}$, where $m \geq 1$.
The high-level idea of our approach is to find the solution using dynamic programming,
in each step extending previously found partial solutions to the vertices of $G'$ corresponding to a next vertex and a next edge of $D'$. 
This is very similar to a dynamic programming using a path decomposition.

For an edge $x_ix_{i+1}$ of $D'$, let $\cL_{i,{i+1}}$ denote the family of all functions $\eta(x_ix_{i+1},x_i) \to V(H)$,
and let $\cR_{i,{i+1}}$ denote the family of all functions from $\eta(x_ix_{i+1},x_{i+1}) \to V(H)$.
Assume now that $i \in \{2,\ldots,m\}$; the first and the last edge will be treated slightly differently.
Recall that the only vertices of $\eta(x_ix_{i+1})$ that might have neighbors outside $\eta(x_ix_{i+1})$
are in $\eta(x_ix_{i+1},x_i)$ and $\eta(x_ix_{i+1},x_{i+1})$. 
We define $\cE_{i,i+1}$ be the set of those pairs $(f,g) \in \cL_{i,i+1} \times \cR_{i,i+1}$,
for which there exists a list homomorphism $h : (G'[\eta(x_ix_{i+1})],L) \to H$,
such that $h|_{\eta(x_ix_{i+1},x_i)} = f$ and $h|_{\eta(x_ix_{i+1},x_{i+1})} = g$.
Note that this condition in particular implies that $f$ and $g$ agree on $\eta(x_ix_{i+1},x_i) \cap \eta(x_ix_{i+1},x_{i+1})$.

Now consider a vertex $x_i$, where $i \in \{2,\ldots,m+1\}$.
Recall that $N_G(\eta(x_i)) \subseteq \eta(x_{i-1}x_i,x_i) \cup \eta(x_ix_{i+1},x_i)$.
By $\cV_i$ we denote the set of those pairs $(f,g) \in \cR_{i-1,i} \times \cL_{i,i+1}$, for which there exists a list homomorphism
$h : (G'[\eta(x_{i-1}x_i,x_i) \cup \eta(x_i) \cup \eta(x_ix_{i+1},x_i)],L) \to H$,
such that $h|_{\eta(x_{i-1}x_{i},x_i)} = f$ and $h|_{\eta(x_ix_{i+1},x_i)} = g$.

Let us describe our dynamic programming. Suppose we have precomputed all sets $\cE_{i,i+1}$ for $i \in \{2,\ldots,m\}$,
and all sets $\cV_i$ for $i \in \{2,\ldots,m+1\}$. 
For each $i \in [m]$, we will compute the set $T[i]$, of those functions in $\cR_{i,i+1}$,
which can be extended to a list homomorphism $(G'[\bigcup_{j \leq i} \left( \eta(x_j) \cup \eta(x_jx_{j+1})\right)],L) \to H$.
Suppose we already have computed the set $T[i]$ and want to extend it to $T[i+1]$.
Then is it easy to observe that $g \in T[i+1]$ if and only if there exist $f \in T[i] \subseteq  \cR_{i,i+1}$ and $f' \in \cL_{i+1,i+2}$,
such that $(f,f') \in \cV_{i+1}$, and $(f',g) \in \cE_{i+1,i+2}$.
Finally, having computed $T[m]$, we report a yes-instance if and only if there exists $f \in T[m]$, which can be extended to a list homomorphism
$(G'[\eta(x_{m}x_{m+1},x_{m+1}) \cup \eta(x_{m+1}) \cup \eta(x_{m+1}x_{m+2}) \cup \eta(x_{m+2})],L)\to H$.

Now let us discuss the complexity of this procedure.
Recall that for each $i \in \{2,\ldots,m\}$, each of sets $\eta(x_ix_{i+1},x_i)$ and $\eta(x_ix_{i+1},x_{i+1})$ has at most $n^{1/9}$ elements. Thus each of sets $\cL_{i,i+1}$ and $\cR_{i,i+1}$ has at most $|V(H)|^{n^{1/9}}$ elements.
A similar bound holds for $\cR_{1,2}$ and $\cL_{m+1,m+2}$.
Furthermore, we can enumerate all sets $\cL_{i,i+1}$ and $\cR_{i,i+1}$, except for $\cL_{1,2}$ and $\cR_{m+1,m+2}$, in total time $\Oh(n \cdot |V(H)|^{n^{1/9}})$.
To compute $\cE_{i,i+1}$ for $i \in \{2,\ldots,m\}$, for each pair $(f,g) \in \cL_{i,i+1} \times \cR_{i,i+1}$, we adjust the lists in $\eta(x_ix_{i+1})$ and solve the obtained instance of \lhomo{H} on the graph $G'[\eta(x_ix_{i+1})]$. By \cref{cor:final-esd}~\cref{it:decomp-size-cor} this graph has at most $\alpha$ vertices, as all its vertices are in one full edge atom. 
So we can compute all sets $\cE_{i,i+1}$ in total time $|V(H)|^{2n^{1/9}} \cdot F(\alpha) \cdot n^{\Oh(1)}$.
Similarly, to compute sets $\cV_i$ for $i \in \{2,\ldots,m\}$, for each pair $(f,g) \in \cR_{i-1,i} \times \cL_{i,i+1}$, we adjust the lists in $\eta(x_i)$ and solve the obtained instance of \lhomo{H} on the graph $G'[\eta(x_i)]$.
Again, by \cref{cor:final-esd}~\cref{it:decomp-size-cor} this graph has at most $\alpha$ vertices.

We compute $T[1]$ as follows. For each $f \in \cR_{1,2}$, we want to verify if $f$ can be extended to list homomorphism $(G'[A],L) \to H$, for $A:=\eta(x_1) \cup \eta(x_1x_2)$. Again, we solve this problem by adjusting the lists of vertices in $A$, and solving an instance of \lhomo{H} on the graph $G'[A]$. By \cref{cor:final-esd}~\cref{it:decomp-size-cor} this instance has at most $\alpha$ vertices.
So we compute $T[1]$ in time $|V(H)|^{n^{1/9}} \cdot F(\alpha) \cdot n^{\Oh(1)}$.

The time needed to extend $T[i]$ to $T[i+1]$ in a way described above is bounded by $|T[i]| \cdot |\cR_{i,i+1}| \cdot |\cL_{i+1,i+2}| \leq |V(H)|^{3n^{1/9}}$.

Finally, having computed $T[m]$, for each $f \in T[m]$ we adjust the list of vertices in $\eta(x_{m+1}) \cup \eta(x_{m+1}x_{m+2},x_{m+1})$
and solve an instance of \lhomo{H} on the subgraph of $G'$ induced by $\eta(x_{m+1}) \cup \eta(x_{m+1}x_{m+2}) \cup \eta(x_{m+2})$. This whole set is contained in the full edge atom of $(D',\eta)$, so its size is at most $\alpha$.
Thus this step can be done in time $|T[m]| \cdot F(\alpha) \cdot n^{\Oh(1)} \leq |V(H)|^{n^{1/9}} \cdot F(\alpha) \cdot n^{\Oh(1)}$.

As $m = \Oh(n)$, we obtain that the total complexity of solving \lhomo{H} on $G'$ in this case is at most $\left(|V(H)|^{2n^{1/9}} F(\alpha) + |V(H)|^{3n^{1/9}}\right) \cdot n^{\Oh(1)} \leq |V(H)|^{4n^{1/9}} F(\alpha) \cdot n^{\Oh(1)}$.

\paragraph{Case 3: $D'$ is a cycle.}
This case can be reduced to the previous one as follows. 
Let the consecutive vertices of $D'$ be $x_1,x_2,\ldots,x_m$.
We exhaustively guess the colors of $\eta(x_1x_2,x_1)$, recall that this set has at most $n^{1/9}$ vertices, so there are at most $|V(H)|^{n^{1/9}}$ possible choices.
We adjust the lists of vertices in $N_G(\eta(x_1x_2,x_1))$, so that they are compatible with the guessed coloring.
Now we want to verify if we can extend the coloring to vertices of $G' \setminus \eta(x_1x_2,x_1)$.
We modify $D'$ by introducing a vertex $x_1'$ and the edge $x_1'x_2$ to $D'$.
We set $\eta(x_1'):=\emptyset$ and $\eta(x_1'x_2,x_1'):=\emptyset$. We also set $\eta(x_1'x_2):=\eta(x_1x_2)$ and $\eta(x_1'x_2,x_2):=\eta(x_1x_2,x_2)$, and we remove the edge $x_1x_2$ from $D'$.
It is straightforward to verify that the modified $(D',\eta)$ is an extended strip decomposition of $G' \setminus \eta(x_1x_2,x_1)$, where $D'$ is a path with $m \geq 3$ edges. Thus we can proceed as in Case 2. The total running time of this step is bounded by 
$|V(H)|^{n^{1/9}} \cdot \left(|V(H)|^{2n^{1/9}} F(\alpha) + |V(H)|^{3n^{1/9}}\right) \cdot n^{\Oh(1)} \leq |V(H)|^{4n^{1/9}} F(\alpha) \cdot n^{\Oh(1)}$.
\end{claimproof}

%-----------
%
%If $D$ is a cycle, we can compute if $G_D \to H$ in time $\left(|H|^{2n^{1/9}} F(\alpha) + |H|^{4n^{1/9}}\right) \cdot \poly(n)$, as we can loop over all possible $H$-colorings of $E^L_1$ and perform an analogous procedure on the remaining part of graph.
%A~total complexity of the algorithm~is 
%\begin{equation}\label{eq:complexity}
%F(n) \leq |H|^{n^{-1/9}(n - \alpha)}\cdot\left(|H|^{2n^{1/9}} F(\alpha) + |H|^{4n^{1/9}}\right) \cdot \poly(n).
%\end{equation}
%---------------

So let us now estimate the total running time of the algorithm in case that the maximum degree of $G$ is at most $n^{1/9}$.
Recall that we exhaustively guess the coloring of $|X|$ and then, for every connected component of $G \setminus X$, we try to extend it, using \cref{cl:extend}.
Thus the overall complexity $F(n)$ in the considered case is described by the following inequality, provided by $n$ is large.
\begin{equation*}
F(n) \leq |V(H)|^{|X|} \cdot |V(H)|^{4n^{1/9}} \cdot F(\alpha) \cdot n^{\Oh(1)} \leq |V(H)|^{|X|} \cdot |V(H)|^{5n^{1/9}} \cdot F(\alpha).
\end{equation*}
By \cref{cor:final-esd}~\cref{it:decomp-sizeX-cor} we have that $|X| \leq n^{-1/9} (n-\alpha)$.
So, applying the inductive assumption, we obtain the bound
\begin{equation}
F(n) \leq  |V(H)|^{ n^{-1/9} (n-\alpha) } \cdot |V(H)|^{5n^{1/9}} \cdot |V(H)|^{a \cdot \alpha^{8/9} \log \alpha}.
\end{equation}
Recall that $1 \leq \alpha \leq n-n^{2/9}$ by \cref{cor:final-esd}~\cref{it:decomp-size-cor}.
In the next claim we show that for these values of $\alpha$, the claimed upper bound holds.

\begin{claim}
If $n$ is sufficiently large and $a \geq 1$, then for every $1 \leq \alpha \leq n - n^{2/9}$ it holds that 
\[
|V(H)|^{ n^{-1/9} (n-\alpha) } \cdot |V(H)|^{5n^{1/9}} \cdot |V(H)|^{a \cdot \alpha^{8/9} \log \alpha} \leq |V(H)|^{a \cdot n^{8/9} \log n}.
\]
\end{claim}
\begin{claimproof}
Note that the statement of the claim is equivalent to showing that
\[
n^{-1/9}(n-\alpha)+5n^{1/9}+a\cdot\alpha^{8/9}\log\alpha \leq a\cdot n^{8/9}\log{n}.
\]

We consider a real function $\psi(x) = n^{-1/9}(n-x)+5n^{1/9}+a\cdot x^{8/9}\log x$,
defined for $x \in [1,n-n^{2/9}]$. Note that $\psi$ is continuous on $[1,n-n^{2/9}]$ and differentiable on $(1,n-n^{2/9})$.
Thus the maximum value of $\psi(x)$ is reached for $x=1$, or $x=n-n^{2/9}$, or for some $x \in (1,n-n^{2/9})$ for which $\psi'(x)=0$.

For $x=1$ observe that if $a \geq 1$, then
$\psi(1)\leq n^{8/9} + 5n^{1/9} \leq a \cdot n^{8/9} \log n$ for sufficiently large $n$.
For $x=n-n^{2/9}$ observe that 
\begin{equation*}
\psi(n-n^{2/9})=6n^{1/9}+a\left(n-n^{2/9}\right)^{8/9}\log\left(n-n^{2/9}\right) \leq a\cdot n^{8/9}\log{n}
\end{equation*}
is equivalent to 
\begin{equation}\label{eq:tone}
\frac{6}{a} \cdot n^{-7/9}+\left(\frac{n-n^{2/9}}{n}\right)^{8/9}\log\left(n-n^{2/9}\right) \leq \log{n}.
\end{equation}

Now we want to use the inequality called \emph{Young's inequality for products}~\cite{mitrinovic1970analytic}:
\begin{equation}\label{young}
\text{For } a,b \geq 0 \text{ and } 0 \leq \theta \leq 1, \text{ it holds that } a^\theta b^{1-\theta} \leq \theta \cdot a + (1-\theta) \cdot b.
\end{equation}

Applying \eqref{young} to the left side of \eqref{eq:tone} gives the following.
\begin{equation*}
\frac{6}{a} \cdot n^{-7/9}+\left(\frac{n-n^{2/9}}{n}\right)^{8/9}\log\left(n-n^{2/9}\right) \leq \frac{6}{a} \cdot n^{-7/9}+\left(\frac{8}{9}\left(1-n^{-7/9}\right) + \frac{1}{9}\right) \log\left(n-n^{2/9}\right).
\end{equation*}
Thus, it is enough to show that 
\begin{equation*}
\frac{6}{a} \cdot n^{-7/9}-\frac{8}{9}n^{-7/9}\log\left(n-n^{2/9}\right) \leq \log\frac{n}{n-n^{2/9}}
\end{equation*}
or, equivalently, 
\begin{equation}\label{eq:ttwo}
\frac{6}{a}-\frac{8}{9}\log\left(n-n^{2/9}\right) \leq n^{7/9}\log\left(1 + \frac{1}{n^{7/9}-1}\right).
\end{equation}
It is straightforward to verify that the left side of \eqref{eq:ttwo} tends to minus infinity when $n \to \infty$ for any $a \geq 1$, while the right side of \eqref{eq:ttwo} is always positive, hence \eqref{eq:ttwo} holds for large $n$.

Finally, $\psi'(x)=-n^{-1/9}+\frac{8}{9}ax^{-1/9}\log x +\frac{ax^{8/9}}{x} = 0$ if and only if $x = na^9\left(\frac{8}{9}\log x+1\right)^9$.
Hence, if $x \leq n-n^{2/9}$, it implies that $na^9\left(\frac{8}{9}\log x+1\right)^9 \leq n-n^{2/9}$.
Since $a^9\left(\frac{8}{9}\log x+1\right)^9 \geq 1$ for $x \geq 1$, this is a contradiction, so there is no $x \in (1,n-n^{2/9})$ for which $\psi'(x)=0$.

Therefore, $\psi(x)\leq  a\cdot n^{8/9}\log{n}$ for every $x \in [1, n-n^{2/9}]$.
Restricting the domain of $\psi$ to integer values of $\alpha$ yields the desired bound.
\end{claimproof} 

This completes the proof of the theorem.
\end{proof}

Combining \cref{thm:subdivided-claw-free-algo} with \cref{thm:factorization}, we immediately obtain the following corollary.

\begin{corollary} \label{cor:subdivided-claw-free-algo-factors}
Let $H$ be a non-predacious graph.
Then for every $a,b,c\geq 0$, the \lhomo{H} problem can be solved in time $2^{\Oh(n^{8/9} \log n)}$ in $n$-vertex $\{S_{a,b,c},K_3\}$-free graphs.
\end{corollary}


\cref{cor:subdivided-claw-free-algo-factors} yields the algorithmic statement in \cref{thm:subdividedclaw-irreflexive}.

\begin{proof}[Proof of \cref{thm:subdividedclaw-irreflexive}~a)]
Observe that since $H$ is irreflexive and triangle-free, there is no homomorphism from $K_3$ to $H$.
Thus if $G$ is not triangle-free, we can immediately report a no-instance.
In the other case, we can use the algorithm from \cref{cor:subdivided-claw-free-algo-factors}.
\end{proof}

